Evaluation of Version Control Merge Tools

A version control system, such as Git, requires a way to integrate changes from different developers or branches. Given a merge scenario, a merge tool either outputs a clean integration of the changes, or it outputs a conflict for manual resolution. A clean integration is correct if it preserves intended program behavior, and is incorrect otherwise (e.g., if it causes a test failure). Manual resolution consumes valuable developer time, and correcting a defect introduced by an incorrect merge is even more costly. New merge tools have been proposed, but they have not yet been evaluated against one another. Prior evaluations do not properly distinguish between correct and incorrect merges, are not evaluated on a realistic set of merge scenarios, and/or do not compare to state-of-the-art tools. We have performed a more realistic evaluation. The results differ significantly from previous claims, setting the record straight and enabling better future research. Our novel experimental methodology combines running test suites, examining merges on deleted branches, and accounting for the cost of incorrect merges. Based on these evaluations, we created a merge tool that out-performs all previous tools under most assumptions. It handles the most common merge scenarios in practice.

==> Makefile <==
# Put user-specific changes in your own Makefile.user.
# Make will silently continue if that file does not exist.
-include Makefile.user

# Mac OS X users may need to add to Makefile.user:
#  LATEXMK = /usr/texbin/latexmk
LATEXMK ?= latexmk

NAME	:= paper

default: all

all: ${NAME}.pdf appendix.pdf

.PRECIOUS: %.pdf
${NAME}.pdf: plume-bib-update
	${LATEXMK} -bibtex -pdf -shell-escape -synctex=1 -interaction=nonstopmode -f "${NAME}.tex"
  # Fail the build if there are undefined references or citations.
	@ ! grep "Warning: There were undefined references." "${NAME}.log"
	@ ! grep "Warning: There were undefined citations." "${NAME}.log"

.PHONY: notodos
notodos: ${NAME}-notodos.pdf
${NAME}-notodos.pdf: ${NAME}.pdf
	pdflatex -shell-escape "\def\notodocomments{}\input{${NAME}}"
	pdflatex -shell-escape "\def\notodocomments{}\input{${NAME}}"
	cp -pf ${NAME}.pdf $@

appendix.pdf: plume-bib-update
	${LATEXMK} -bibtex -pdf -shell-escape -synctex=1 -interaction=nonstopmode -f appendix.tex
  # Fail the build if there are undefined references or citations.
	@ ! grep "Warning: There were undefined references." appendix.log
	@ ! grep "Warning: There were undefined citations." appendix.log

# You will upload onefile.zip to the publisher website after acceptance.
onefile.zip: onefile.tex
	zip onefile.zip onefile.tex acmart.cls ACM-Reference-Format.bst
# The latex-process-inputs program is part of https://github.com/plume-lib/plume-scripts .
onefile.tex:
	latex-process-inputs ${NAME}.tex > onefile.tex


# You will upload appendix-onefile.zip to the arXiv.
appendix-onefile.zip: appendix-onefile.tex
	zip appendix-onefile.zip appendix-onefile.tex acmart.cls ACM-Reference-Format.bst
# The latex-process-inputs program is part of https://github.com/plume-lib/plume-scripts .
appendix-onefile.tex:
	latex-process-inputs ${NAME}.tex > appendix-onefile.tex

appendix-onefile.tex: appendix.tex


# This target creates:
#   https://homes.cs.washington.edu/~mernst/tmp72112/ast-merging.pdf
web: ${NAME}-notodos.pdf
	cp -pf $^ ${HOME}/public_html/tmp72112/ast-merging.pdf

view: ${NAME}.pdf
	open $<

ispell: spell
spell:
	for file in `latex-process-inputs -list ${NAME}.tex`; do ispell $$file; done

# Count words in the abstract, which some conferences limit.
abs-words:
	grep -v 'Abstract' abstract.tex | egrep -v '^%' | wc -w

plume-bib:
ifdef PLUMEBIB
	ln -s ${PLUMEBIB} $@
else
	git clone https://github.com/mernst/plume-bib.git
endif
.PHONY: plume-bib-update
# Even if the plume-bib-update target fails, it does not terminate the make job.
# However, to skip it, invoke make as:  make NOGIT=1 ...
plume-bib-update: plume-bib
ifndef NOGIT
	-(cd plume-bib && GIT_TERMINAL_PROMPT=0 git -c credential.helper= pull && make)
endif

.PHONY: tags
TAGS: tags
tags:
	etags `latex-process-inputs -list ${NAME}.tex` `latex-process-inputs -list appendix.tex`

clean:
	${LATEXMK} -C "${NAME}.tex"


==> results/combined/tables/all/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-ort-ignorespace         &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Gitmerge-recursive-histogram     &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-recursive-myers-ignorespace &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Gitmerge-recursive-minimal       &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-recursive-myers         &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-recursive-patience      &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-resolve                 &  52\% &  35\% &  45\% &  63\% &   3\% &   2\% \\
            Hires-Merge                      &  57\% &  41\% &  39\% &  55\% &   4\% &   4\% \\
            Spork                            &  62\% &  44\% &  28\% &  45\% &  11\% &  11\% \\
            IntelliMerge                     &  27\% &  19\% &  21\% &  34\% &  52\% &  47\% \\
            Adjacent                         &  58\% &  42\% &  39\% &  54\% &   4\% &   4\% \\
            Imports                          &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Version Numbers                  &  54\% &  36\% &  44\% &  61\% &   3\% &   2\% \\
            IVn                              &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            IVn-ignorespace                  &  59\% &  42\% &  38\% &  54\% &   3\% &   4\% \\
            Gitmerge-ort-plus                &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Gitmerge-ort-ignorespace-plus    &  59\% &  42\% &  38\% &  54\% &   3\% &   4\% \\
            Gitmerge-recursive-histogram-plus &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Gitmerge-recursive-myers-ignorespace-plus &  59\% &  42\% &  38\% &  54\% &   3\% &   4\% \\
            Gitmerge-recursive-minimal-plus  &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Gitmerge-recursive-myers-plus    &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Gitmerge-recursive-patience-plus &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Gitmerge-resolve-plus            &  56\% &  40\% &  41\% &  57\% &   3\% &   3\% \\
            Git-hires-merge-plus             &  61\% &  46\% &  35\% &  50\% &   4\% &   4\% \\
            Spork-plus                       &  63\% &  47\% &  26\% &  42\% &  11\% &  11\% \\
            Intellimerge-plus                &   8\% &   9\% &  21\% &  33\% &  71\% &  58\% \\
            Adjacent-plus                    &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Imports-plus                     &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Version-numbers-plus             &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Ivn-plus                         &  57\% &  41\% &  40\% &  57\% &   3\% &   3\% \\
            Ivn-ignorespace-plus             &  59\% &  42\% &  38\% &  54\% &   3\% &   4\% \\
\end{tabular}


==> results/combined/tables/all/table_run_time.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{c|c|c|c}
    & \multicolumn{3}{c}{Run time (seconds)} \\
    Tool & Mean & Median & Max \\
    \hline
    Gitmerge-ort                     & 0.04 & 0.04 & 1.19 \\
    Gitmerge-ort-ignorespace         & 0.04 & 0.04 & 1.22 \\
    Gitmerge-recursive-histogram     & 0.05 & 0.04 & 2.97 \\
    Gitmerge-recursive-myers-ignorespace & 0.03 & 0.02 & 2.17 \\
    Gitmerge-recursive-minimal       & 0.05 & 0.04 & 2.13 \\
    Gitmerge-recursive-myers         & 0.05 & 0.04 & 2.11 \\
    Gitmerge-recursive-patience      & 0.05 & 0.04 & 3.05 \\
    Gitmerge-resolve                 & 0.24 & 0.17 & 5.02 \\
    Hires-Merge                      & 0.23 & 0.13 & 17.3 \\
    Spork                            & 2.55 & 1.06 & 653 \\
    IntelliMerge                     & 1.04 & 0.50 & 89.3 \\
    Adjacent                         & 0.17 & 0.05 & 76.9 \\
    Imports                          & 0.11 & 0.07 & 7.86 \\
    Version Numbers                  & 0.07 & 0.05 & 2.75 \\
    IVn                              & 0.12 & 0.08 & 7.97 \\
    IVn-ignorespace                  & 0.12 & 0.08 & 8.08 \\
    Gitmerge-ort-plus                & 0.12 & 0.07 & 7.56 \\
    Gitmerge-ort-ignorespace-plus    & 0.11 & 0.07 & 7.42 \\
    Gitmerge-recursive-histogram-plus & 0.12 & 0.07 & 7.54 \\
    Gitmerge-recursive-myers-ignorespace-plus & 0.12 & 0.08 & 7.63 \\
    Gitmerge-recursive-minimal-plus  & 0.12 & 0.07 & 7.53 \\
    Gitmerge-recursive-myers-plus    & 0.12 & 0.08 & 7.48 \\
    Gitmerge-recursive-patience-plus & 0.12 & 0.07 & 7.61 \\
    Gitmerge-resolve-plus            & 0.19 & 0.12 & 13.6 \\
    Git-hires-merge-plus             & 0.21 & 0.13 & 14.8 \\
    Spork-plus                       & 2.67 & 1.13 & 600 \\
    Intellimerge-plus                & 1.13 & 0.57 & 91.8 \\
    Adjacent-plus                    & 0.12 & 0.07 & 7.46 \\
    Imports-plus                     & 0.12 & 0.07 & 7.43 \\
    Version-numbers-plus             & 0.12 & 0.07 & 7.44 \\
    Ivn-plus                         & 0.12 & 0.07 & 7.51 \\
    Ivn-ignorespace-plus             & 0.11 & 0.07 & 7.52 \\
\end{tabular}


==> results/combined/tables/all/table_summary.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{l|c c|c c|c c|}
        Tool & \multicolumn{6}{c|}{Merges} \\ \cline{2-7}
        & \multicolumn{2}{c|}{Correct} &
        \multicolumn{2}{c|}{Unhandled} &
        \multicolumn{2}{c|}{Incorrect} \\
        & \# & \% & \# & \% & \# & \% \\
        \hline
Gitmerge-ort                     &  2748 &  46\% &  3078 &  51\% &   157 &   3\% \\
Gitmerge-ort-ignorespace         &  2889 &  48\% &  2905 &  49\% &   189 &   3\% \\
Gitmerge-recursive-histogram     &  2748 &  46\% &  3078 &  51\% &   157 &   3\% \\
Gitmerge-recursive-myers-ignorespace &  2890 &  48\% &  2902 &  49\% &   191 &   3\% \\
Gitmerge-recursive-minimal       &  2748 &  46\% &  3078 &  51\% &   157 &   3\% \\
Gitmerge-recursive-myers         &  2748 &  46\% &  3078 &  51\% &   157 &   3\% \\
Gitmerge-recursive-patience      &  2751 &  46\% &  3074 &  51\% &   158 &   3\% \\
Gitmerge-resolve                 &  2703 &  45\% &  3124 &  52\% &   156 &   3\% \\
Hires-Merge                      &  3040 &  51\% &  2721 &  45\% &   222 &   4\% \\
Spork                            &  3260 &  54\% &  2080 &  35\% &   643 &  11\% \\
IntelliMerge                     &  1434 &  24\% &  1582 &  26\% &  2967 &  50\% \\
Adjacent                         &  3073 &  51\% &  2692 &  45\% &   218 &   4\% \\
Imports                          &  2904 &  49\% &  2910 &  49\% &   169 &   3\% \\
Version Numbers                  &  2782 &  46\% &  3044 &  51\% &   157 &   3\% \\
IVn                              &  3011 &  50\% &  2803 &  47\% &   169 &   3\% \\
IVn-ignorespace                  &  3116 &  52\% &  2665 &  45\% &   202 &   3\% \\
Gitmerge-ort-plus                &  3011 &  50\% &  2803 &  47\% &   169 &   3\% \\
Gitmerge-ort-ignorespace-plus    &  3116 &  52\% &  2665 &  45\% &   202 &   3\% \\
Gitmerge-recursive-histogram-plus &  3011 &  50\% &  2803 &  47\% &   169 &   3\% \\
Gitmerge-recursive-myers-ignorespace-plus &  3116 &  52\% &  2664 &  45\% &   203 &   3\% \\
Gitmerge-recursive-minimal-plus  &  3012 &  50\% &  2802 &  47\% &   169 &   3\% \\
Gitmerge-recursive-myers-plus    &  3012 &  50\% &  2802 &  47\% &   169 &   3\% \\
Gitmerge-recursive-patience-plus &  3013 &  50\% &  2801 &  47\% &   169 &   3\% \\
Gitmerge-resolve-plus            &  2974 &  50\% &  2843 &  48\% &   166 &   3\% \\
Git-hires-merge-plus             &  3274 &  55\% &  2473 &  41\% &   236 &   4\% \\
Spork-plus                       &  3392 &  57\% &  1937 &  32\% &   654 &  11\% \\
Intellimerge-plus                &   497 &   8\% &  1552 &  26\% &  3934 &  66\% \\
Adjacent-plus                    &  3011 &  50\% &  2803 &  47\% &   169 &   3\% \\
Imports-plus                     &  3011 &  50\% &  2803 &  47\% &   169 &   3\% \\
Version-numbers-plus             &  3011 &  50\% &  2803 &  47\% &   169 &   3\% \\
Ivn-plus                         &  3011 &  50\% &  2803 &  47\% &   169 &   3\% \\
Ivn-ignorespace-plus             &  3116 &  52\% &  2665 &  45\% &   202 &   3\% \\
\end{tabular}


==> results/combined/tables/all/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Gitmerge-recursive-histogram & Gitmerge-recursive-myers-ignorespace & Gitmerge-recursive-minimal & Gitmerge-recursive-myers & Gitmerge-recursive-patience & Gitmerge-resolve & Hires-Merge & Spork & IntelliMerge & Adjacent & Imports & Version Numbers & IVn & IVn-ignorespace & Gitmerge-ort-plus & Gitmerge-ort-ignorespace-plus & Gitmerge-recursive-histogram-plus & Gitmerge-recursive-myers-ignorespace-plus & Gitmerge-recursive-minimal-plus & Gitmerge-recursive-myers-plus & Gitmerge-recursive-patience-plus & Gitmerge-resolve-plus & Git-hires-merge-plus & Spork-plus & Intellimerge-plus & Adjacent-plus & Imports-plus & Version-numbers-plus & Ivn-plus & Ivn-ignorespace-plus \\
\midrule
Gitmerge-ort & - & 2 & 0 & 3 & 1 & 1 & 0 & 3 & 1 & 5 & 8 & 0 & 0 & 0 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 13 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-ort-ignorespace & 27 & - & 27 & 1 & 28 & 28 & 27 & 30 & 22 & 20 & 18 & 19 & 27 & 27 & 26 & 0 & 26 & 0 & 26 & 0 & 26 & 26 & 26 & 28 & 19 & 18 & 24 & 26 & 26 & 26 & 26 & 0 \\
Gitmerge-recursive-histogram & 0 & 2 & - & 3 & 1 & 1 & 0 & 3 & 1 & 5 & 8 & 0 & 0 & 0 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 13 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-recursive-myers-ignorespace & 29 & 1 & 29 & - & 28 & 28 & 28 & 31 & 22 & 22 & 18 & 21 & 27 & 29 & 26 & 0 & 26 & 0 & 26 & 0 & 26 & 26 & 26 & 29 & 19 & 19 & 24 & 26 & 26 & 26 & 26 & 0 \\
Gitmerge-recursive-minimal & 1 & 3 & 1 & 2 & - & 0 & 0 & 2 & 0 & 5 & 8 & 1 & 0 & 1 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 13 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-recursive-myers & 1 & 3 & 1 & 2 & 0 & - & 0 & 2 & 0 & 5 & 8 & 1 & 0 & 1 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 13 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-recursive-patience & 1 & 3 & 1 & 3 & 1 & 1 & - & 3 & 1 & 5 & 8 & 1 & 0 & 1 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 13 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-resolve & 2 & 4 & 2 & 3 & 1 & 1 & 1 & - & 1 & 6 & 9 & 2 & 1 & 2 & 1 & 3 & 1 & 3 & 1 & 3 & 1 & 1 & 1 & 0 & 1 & 4 & 14 & 1 & 1 & 1 & 1 & 3 \\
Hires-Merge & 66 & 61 & 66 & 60 & 65 & 65 & 65 & 67 & - & 33 & 28 & 43 & 65 & 65 & 62 & 57 & 62 & 57 & 62 & 57 & 62 & 62 & 62 & 65 & 0 & 27 & 32 & 62 & 62 & 62 & 62 & 57 \\
Spork & 289 & 268 & 289 & 268 & 289 & 289 & 286 & 295 & 237 & - & 73 & 233 & 258 & 285 & 250 & 227 & 250 & 227 & 250 & 226 & 249 & 249 & 248 & 255 & 197 & 0 & 79 & 250 & 250 & 250 & 250 & 227 \\
IntelliMerge & 1546 & 1436 & 1546 & 1435 & 1545 & 1545 & 1540 & 1562 & 1293 & 740 & - & 1265 & 1415 & 1545 & 1365 & 1282 & 1365 & 1282 & 1365 & 1283 & 1363 & 1363 & 1361 & 1384 & 1133 & 680 & 5 & 1365 & 1365 & 1365 & 1365 & 1282 \\
Adjacent & 61 & 56 & 61 & 57 & 62 & 62 & 60 & 64 & 39 & 32 & 23 & - & 55 & 61 & 54 & 49 & 54 & 49 & 54 & 49 & 54 & 54 & 53 & 56 & 31 & 28 & 27 & 54 & 54 & 54 & 54 & 49 \\
Imports & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & - & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & 0 & 0 & 0 & 0 & 1 \\
Version Numbers & 0 & 2 & 0 & 3 & 1 & 1 & 0 & 3 & 1 & 5 & 8 & 0 & 0 & - & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 13 & 0 & 0 & 0 & 0 & 2 \\
IVn & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & - & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & 0 & 0 & 0 & 0 & 1 \\
IVn-ignorespace & 27 & 0 & 27 & 2 & 28 & 28 & 27 & 32 & 22 & 22 & 22 & 20 & 27 & 27 & 26 & - & 26 & 0 & 26 & 1 & 26 & 26 & 26 & 30 & 19 & 19 & 28 & 26 & 26 & 26 & 26 & 0 \\
Gitmerge-ort-plus & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & - & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-ort-ignorespace-plus & 27 & 0 & 27 & 2 & 28 & 28 & 27 & 32 & 22 & 22 & 22 & 20 & 27 & 27 & 26 & 0 & 26 & - & 26 & 1 & 26 & 26 & 26 & 30 & 19 & 19 & 28 & 26 & 26 & 26 & 26 & 0 \\
Gitmerge-recursive-histogram-plus & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & - & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-myers-ignorespace-plus & 29 & 1 & 29 & 0 & 28 & 28 & 29 & 33 & 22 & 24 & 22 & 22 & 28 & 29 & 27 & 1 & 27 & 1 & 27 & - & 26 & 26 & 27 & 31 & 19 & 20 & 28 & 27 & 27 & 27 & 27 & 1 \\
Gitmerge-recursive-minimal-plus & 1 & 2 & 1 & 2 & 0 & 0 & 1 & 4 & 0 & 8 & 12 & 1 & 1 & 1 & 1 & 2 & 1 & 2 & 1 & 2 & - & 0 & 1 & 4 & 0 & 5 & 17 & 1 & 1 & 1 & 1 & 2 \\
Gitmerge-recursive-myers-plus & 1 & 2 & 1 & 2 & 0 & 0 & 1 & 4 & 0 & 8 & 12 & 1 & 1 & 1 & 1 & 2 & 1 & 2 & 1 & 2 & 0 & - & 1 & 4 & 0 & 5 & 17 & 1 & 1 & 1 & 1 & 2 \\
Gitmerge-recursive-patience-plus & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & - & 4 & 0 & 4 & 17 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-resolve-plus & 2 & 3 & 2 & 3 & 1 & 1 & 2 & 0 & 1 & 9 & 12 & 2 & 2 & 2 & 2 & 3 & 2 & 3 & 2 & 3 & 1 & 1 & 2 & - & 1 & 6 & 17 & 2 & 2 & 2 & 2 & 3 \\
Git-hires-merge-plus & 68 & 61 & 68 & 61 & 67 & 67 & 68 & 71 & 0 & 37 & 32 & 42 & 68 & 67 & 65 & 58 & 65 & 58 & 65 & 58 & 64 & 64 & 65 & 69 & - & 30 & 36 & 65 & 65 & 65 & 65 & 58 \\
Spork-plus & 293 & 270 & 293 & 271 & 294 & 294 & 291 & 301 & 240 & 0 & 78 & 238 & 270 & 289 & 263 & 237 & 263 & 237 & 263 & 236 & 262 & 262 & 261 & 269 & 208 & - & 84 & 263 & 263 & 263 & 263 & 237 \\
Intellimerge-plus & 1544 & 1439 & 1544 & 1438 & 1544 & 1544 & 1539 & 1579 & 1298 & 757 & 0 & 1263 & 1413 & 1543 & 1364 & 1286 & 1364 & 1286 & 1364 & 1287 & 1363 & 1363 & 1361 & 1395 & 1136 & 695 & - & 1364 & 1364 & 1364 & 1364 & 1286 \\
Adjacent-plus & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & - & 0 & 0 & 0 & 1 \\
Imports-plus & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & 0 & - & 0 & 0 & 1 \\
Version-numbers-plus & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & 0 & 0 & - & 0 & 1 \\
Ivn-plus & 0 & 1 & 0 & 3 & 1 & 1 & 0 & 5 & 1 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 17 & 0 & 0 & 0 & - & 1 \\
Ivn-ignorespace-plus & 27 & 0 & 27 & 2 & 28 & 28 & 27 & 32 & 22 & 22 & 22 & 20 & 27 & 27 & 26 & 0 & 26 & 0 & 26 & 1 & 26 & 26 & 26 & 30 & 19 & 19 & 28 & 26 & 26 & 26 & 26 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/combined/tables/git/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-ort-ignorespace         &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Gitmerge-recursive-histogram     &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-recursive-minimal       &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-recursive-myers         &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-recursive-patience      &  53\% &  35\% &  44\% &  62\% &   3\% &   2\% \\
            Gitmerge-resolve                 &  52\% &  35\% &  45\% &  63\% &   3\% &   2\% \\
\end{tabular}


==> results/combined/tables/git/table_run_time.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{c|c|c|c}
    & \multicolumn{3}{c}{Run time (seconds)} \\
    Tool & Mean & Median & Max \\
    \hline
    Gitmerge-ort                     & 0.04 & 0.04 & 1.19 \\
    Gitmerge-ort-ignorespace         & 0.04 & 0.04 & 1.22 \\
    Gitmerge-recursive-histogram     & 0.05 & 0.04 & 2.97 \\
    Gitmerge-recursive-minimal       & 0.05 & 0.04 & 2.13 \\
    Gitmerge-recursive-myers         & 0.05 & 0.04 & 2.11 \\
    Gitmerge-recursive-patience      & 0.05 & 0.04 & 3.05 \\
    Gitmerge-resolve                 & 0.24 & 0.17 & 5.02 \\
\end{tabular}


==> results/combined/tables/git/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Gitmerge-recursive-histogram & Gitmerge-recursive-minimal & Gitmerge-recursive-myers & Gitmerge-recursive-patience & Gitmerge-resolve \\
\midrule
Gitmerge-ort & - & 2 & 0 & 1 & 1 & 0 & 3 \\
Gitmerge-ort-ignorespace & 27 & - & 27 & 28 & 28 & 27 & 30 \\
Gitmerge-recursive-histogram & 0 & 2 & - & 1 & 1 & 0 & 3 \\
Gitmerge-recursive-minimal & 1 & 3 & 1 & - & 0 & 0 & 2 \\
Gitmerge-recursive-myers & 1 & 3 & 1 & 0 & - & 0 & 2 \\
Gitmerge-recursive-patience & 1 & 3 & 1 & 1 & 1 & - & 3 \\
Gitmerge-resolve & 2 & 4 & 2 & 1 & 1 & 1 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/combined/tables/tools/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Hires-Merge & Spork & IntelliMerge & Adjacent & Imports & Version Numbers & IVn & IVn-ignorespace \\
\midrule
Gitmerge-ort & - & 2 & 1 & 5 & 8 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-ort-ignorespace & 27 & - & 22 & 20 & 18 & 19 & 27 & 27 & 26 & 0 \\
Hires-Merge & 66 & 61 & - & 33 & 28 & 43 & 65 & 65 & 62 & 57 \\
Spork & 289 & 268 & 237 & - & 73 & 233 & 258 & 285 & 250 & 227 \\
IntelliMerge & 1546 & 1436 & 1293 & 740 & - & 1265 & 1415 & 1545 & 1365 & 1282 \\
Adjacent & 61 & 56 & 39 & 32 & 23 & - & 55 & 61 & 54 & 49 \\
Imports & 0 & 1 & 1 & 7 & 12 & 0 & - & 0 & 0 & 1 \\
Version Numbers & 0 & 2 & 1 & 5 & 8 & 0 & 0 & - & 0 & 2 \\
IVn & 0 & 1 & 1 & 7 & 12 & 0 & 0 & 0 & - & 1 \\
IVn-ignorespace & 27 & 0 & 22 & 22 & 22 & 20 & 27 & 27 & 26 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/greatest_hits/tables/all/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-ort-ignorespace         &  55\% &  34\% &  41\% &  63\% &   4\% &   3\% \\
            Gitmerge-recursive-histogram     &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-recursive-myers-ignorespace &  55\% &  34\% &  41\% &  63\% &   4\% &   3\% \\
            Gitmerge-recursive-minimal       &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-recursive-myers         &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-recursive-patience      &  54\% &  32\% &  42\% &  65\% &   4\% &   2\% \\
            Gitmerge-resolve                 &  53\% &  32\% &  43\% &  66\% &   4\% &   2\% \\
            Hires-Merge                      &  59\% &  40\% &  36\% &  56\% &   6\% &   4\% \\
            Spork                            &  58\% &  44\% &  26\% &  50\% &  16\% &   6\% \\
            IntelliMerge                     &  25\% &  15\% &  19\% &  40\% &  56\% &  46\% \\
            Adjacent                         &  59\% &  40\% &  36\% &  57\% &   6\% &   3\% \\
            Imports                          &  57\% &  35\% &  39\% &  62\% &   4\% &   3\% \\
            Version Numbers                  &  54\% &  32\% &  41\% &  65\% &   4\% &   2\% \\
            IVn                              &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            IVn-ignorespace                  &  59\% &  37\% &  38\% &  59\% &   3\% &   4\% \\
            Gitmerge-ort-plus                &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Gitmerge-ort-ignorespace-plus    &  59\% &  37\% &  38\% &  59\% &   3\% &   4\% \\
            Gitmerge-recursive-histogram-plus &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Gitmerge-recursive-myers-ignorespace-plus &  59\% &  37\% &  38\% &  59\% &   3\% &   4\% \\
            Gitmerge-recursive-minimal-plus  &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Gitmerge-recursive-myers-plus    &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Gitmerge-recursive-patience-plus &  58\% &  37\% &  38\% &  60\% &   4\% &   3\% \\
            Gitmerge-resolve-plus            &  57\% &  36\% &  39\% &  61\% &   4\% &   3\% \\
            Git-hires-merge-plus             &  62\% &  43\% &  33\% &  52\% &   5\% &   5\% \\
            Spork-plus                       &  60\% &  45\% &  25\% &  48\% &  15\% &   7\% \\
            Intellimerge-plus                &   5\% &   5\% &  20\% &  40\% &  76\% &  55\% \\
            Adjacent-plus                    &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Imports-plus                     &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Version-numbers-plus             &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Ivn-plus                         &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            Ivn-ignorespace-plus             &  59\% &  37\% &  38\% &  59\% &   3\% &   4\% \\
\end{tabular}


==> results/greatest_hits/tables/all/table_summary.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{l|c c|c c|c c|}
        Tool & \multicolumn{6}{c|}{Merges} \\ \cline{2-7}
        & \multicolumn{2}{c|}{Correct} &
        \multicolumn{2}{c|}{Unhandled} &
        \multicolumn{2}{c|}{Incorrect} \\
        & \# & \% & \# & \% & \# & \% \\
        \hline
Gitmerge-ort                     &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-ort-ignorespace         &   499 &  43\% &   612 &  53\% &    38 &   3\% \\
Gitmerge-recursive-histogram     &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-recursive-myers-ignorespace &   499 &  43\% &   612 &  53\% &    38 &   3\% \\
Gitmerge-recursive-minimal       &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-recursive-myers         &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-recursive-patience      &   484 &  42\% &   629 &  55\% &    36 &   3\% \\
Gitmerge-resolve                 &   475 &  41\% &   640 &  56\% &    34 &   3\% \\
Hires-Merge                      &   554 &  48\% &   541 &  47\% &    54 &   5\% \\
Spork                            &   579 &  50\% &   451 &  39\% &   119 &  10\% \\
IntelliMerge                     &   223 &  19\% &   347 &  30\% &   579 &  50\% \\
Adjacent                         &   556 &  48\% &   542 &  47\% &    51 &   4\% \\
Imports                          &   512 &  45\% &   597 &  52\% &    40 &   3\% \\
Version Numbers                  &   487 &  42\% &   627 &  55\% &    35 &   3\% \\
IVn                              &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
IVn-ignorespace                  &   540 &  47\% &   565 &  49\% &    44 &   4\% \\
Gitmerge-ort-plus                &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
Gitmerge-ort-ignorespace-plus    &   540 &  47\% &   565 &  49\% &    44 &   4\% \\
Gitmerge-recursive-histogram-plus &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
Gitmerge-recursive-myers-ignorespace-plus &   541 &  47\% &   565 &  49\% &    43 &   4\% \\
Gitmerge-recursive-minimal-plus  &   531 &  46\% &   579 &  50\% &    39 &   3\% \\
Gitmerge-recursive-myers-plus    &   531 &  46\% &   579 &  50\% &    39 &   3\% \\
Gitmerge-recursive-patience-plus &   531 &  46\% &   578 &  50\% &    40 &   3\% \\
Gitmerge-resolve-plus            &   522 &  45\% &   589 &  51\% &    38 &   3\% \\
Git-hires-merge-plus             &   598 &  52\% &   495 &  43\% &    56 &   5\% \\
Spork-plus                       &   596 &  52\% &   431 &  38\% &   122 &  11\% \\
Intellimerge-plus                &    56 &   5\% &   354 &  31\% &   739 &  64\% \\
Adjacent-plus                    &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
Imports-plus                     &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
Version-numbers-plus             &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
Ivn-plus                         &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
Ivn-ignorespace-plus             &   540 &  47\% &   565 &  49\% &    44 &   4\% \\
\end{tabular}


==> results/greatest_hits/tables/all/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Gitmerge-recursive-histogram & Gitmerge-recursive-myers-ignorespace & Gitmerge-recursive-minimal & Gitmerge-recursive-myers & Gitmerge-recursive-patience & Gitmerge-resolve & Hires-Merge & Spork & IntelliMerge & Adjacent & Imports & Version Numbers & IVn & IVn-ignorespace & Gitmerge-ort-plus & Gitmerge-ort-ignorespace-plus & Gitmerge-recursive-histogram-plus & Gitmerge-recursive-myers-ignorespace-plus & Gitmerge-recursive-minimal-plus & Gitmerge-recursive-myers-plus & Gitmerge-recursive-patience-plus & Gitmerge-resolve-plus & Git-hires-merge-plus & Spork-plus & Intellimerge-plus & Adjacent-plus & Imports-plus & Version-numbers-plus & Ivn-plus & Ivn-ignorespace-plus \\
\midrule
Gitmerge-ort & - & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-ort-ignorespace & 6 & - & 6 & 1 & 7 & 7 & 6 & 8 & 5 & 3 & 1 & 5 & 6 & 6 & 5 & 0 & 5 & 0 & 5 & 0 & 5 & 5 & 5 & 6 & 3 & 3 & 2 & 5 & 5 & 5 & 5 & 0 \\
Gitmerge-recursive-histogram & 0 & 1 & - & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-myers-ignorespace & 7 & 1 & 7 & - & 6 & 6 & 6 & 7 & 4 & 3 & 1 & 6 & 6 & 7 & 5 & 0 & 5 & 0 & 5 & 0 & 5 & 5 & 5 & 6 & 3 & 3 & 2 & 5 & 5 & 5 & 5 & 0 \\
Gitmerge-recursive-minimal & 1 & 2 & 1 & 1 & - & 0 & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-myers & 1 & 2 & 1 & 1 & 0 & - & 0 & 1 & 0 & 0 & 1 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-patience & 1 & 2 & 1 & 2 & 1 & 1 & - & 2 & 1 & 0 & 1 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-resolve & 1 & 2 & 1 & 1 & 0 & 0 & 0 & - & 0 & 0 & 1 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 1 \\
Hires-Merge & 20 & 18 & 20 & 17 & 19 & 19 & 19 & 20 & - & 9 & 9 & 13 & 19 & 20 & 19 & 17 & 19 & 17 & 19 & 17 & 19 & 19 & 19 & 20 & 0 & 9 & 10 & 19 & 19 & 19 & 19 & 17 \\
Spork & 48 & 46 & 48 & 46 & 48 & 48 & 47 & 50 & 38 & - & 8 & 34 & 41 & 48 & 41 & 39 & 41 & 39 & 41 & 39 & 41 & 41 & 41 & 43 & 31 & 0 & 12 & 41 & 41 & 41 & 41 & 39 \\
IntelliMerge & 313 & 300 & 313 & 300 & 313 & 313 & 312 & 317 & 262 & 157 & - & 253 & 283 & 313 & 273 & 263 & 273 & 263 & 273 & 263 & 273 & 273 & 273 & 278 & 223 & 149 & 1 & 273 & 273 & 273 & 273 & 263 \\
Adjacent & 16 & 16 & 16 & 17 & 17 & 17 & 16 & 18 & 10 & 7 & 4 & - & 16 & 16 & 15 & 15 & 15 & 15 & 15 & 15 & 15 & 15 & 15 & 16 & 8 & 7 & 4 & 15 & 15 & 15 & 15 & 15 \\
Imports & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & - & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
Version Numbers & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 1 & 0 & 0 & - & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 1 \\
IVn & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & - & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
IVn-ignorespace & 7 & 0 & 7 & 1 & 8 & 8 & 7 & 9 & 6 & 4 & 4 & 6 & 7 & 7 & 6 & - & 6 & 0 & 6 & 0 & 6 & 6 & 6 & 7 & 4 & 4 & 5 & 6 & 6 & 6 & 6 & 0 \\
Gitmerge-ort-plus & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & - & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-ort-ignorespace-plus & 7 & 0 & 7 & 1 & 8 & 8 & 7 & 9 & 6 & 4 & 4 & 6 & 7 & 7 & 6 & 0 & 6 & - & 6 & 0 & 6 & 6 & 6 & 7 & 4 & 4 & 5 & 6 & 6 & 6 & 6 & 0 \\
Gitmerge-recursive-histogram-plus & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & - & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-myers-ignorespace-plus & 7 & 0 & 7 & 0 & 7 & 7 & 7 & 8 & 5 & 4 & 4 & 6 & 7 & 7 & 6 & 0 & 6 & 0 & 6 & - & 6 & 6 & 6 & 7 & 4 & 4 & 5 & 6 & 6 & 6 & 6 & 0 \\
Gitmerge-recursive-minimal-plus & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & - & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-myers-plus & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & - & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-patience-plus & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & - & 1 & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-resolve-plus & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & - & 0 & 0 & 4 & 0 & 0 & 0 & 0 & 1 \\
Git-hires-merge-plus & 17 & 15 & 17 & 15 & 17 & 17 & 17 & 18 & 0 & 8 & 10 & 11 & 17 & 17 & 17 & 15 & 17 & 15 & 17 & 15 & 17 & 17 & 17 & 18 & - & 8 & 11 & 17 & 17 & 17 & 17 & 15 \\
Spork-plus & 46 & 44 & 46 & 45 & 47 & 47 & 46 & 49 & 37 & 0 & 10 & 33 & 40 & 46 & 40 & 38 & 40 & 38 & 40 & 38 & 40 & 40 & 40 & 42 & 30 & - & 14 & 40 & 40 & 40 & 40 & 38 \\
Intellimerge-plus & 312 & 300 & 312 & 300 & 312 & 312 & 311 & 320 & 261 & 159 & 0 & 252 & 282 & 312 & 273 & 264 & 273 & 264 & 273 & 264 & 273 & 273 & 273 & 282 & 223 & 151 & - & 273 & 273 & 273 & 273 & 264 \\
Adjacent-plus & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & - & 0 & 0 & 0 & 1 \\
Imports-plus & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & - & 0 & 0 & 1 \\
Version-numbers-plus & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & - & 0 & 1 \\
Ivn-plus & 0 & 1 & 0 & 2 & 1 & 1 & 0 & 2 & 1 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 & - & 1 \\
Ivn-ignorespace-plus & 7 & 0 & 7 & 1 & 8 & 8 & 7 & 9 & 6 & 4 & 4 & 6 & 7 & 7 & 6 & 0 & 6 & 0 & 6 & 0 & 6 & 6 & 6 & 7 & 4 & 4 & 5 & 6 & 6 & 6 & 6 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/greatest_hits/tables/git/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-ort-ignorespace         &  55\% &  34\% &  41\% &  63\% &   4\% &   3\% \\
            Gitmerge-recursive-histogram     &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-recursive-minimal       &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-recursive-myers         &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-recursive-patience      &  54\% &  32\% &  42\% &  65\% &   4\% &   2\% \\
            Gitmerge-resolve                 &  53\% &  32\% &  43\% &  66\% &   4\% &   2\% \\
\end{tabular}


==> results/greatest_hits/tables/git/table_summary.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{l|c c|c c|c c|}
        Tool & \multicolumn{6}{c|}{Merges} \\ \cline{2-7}
        & \multicolumn{2}{c|}{Correct} &
        \multicolumn{2}{c|}{Unhandled} &
        \multicolumn{2}{c|}{Incorrect} \\
        & \# & \% & \# & \% & \# & \% \\
        \hline
Gitmerge-ort                     &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-ort-ignorespace         &   499 &  43\% &   612 &  53\% &    38 &   3\% \\
Gitmerge-recursive-histogram     &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-recursive-minimal       &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-recursive-myers         &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-recursive-patience      &   484 &  42\% &   629 &  55\% &    36 &   3\% \\
Gitmerge-resolve                 &   475 &  41\% &   640 &  56\% &    34 &   3\% \\
\end{tabular}


==> results/greatest_hits/tables/git/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Gitmerge-recursive-histogram & Gitmerge-recursive-minimal & Gitmerge-recursive-myers & Gitmerge-recursive-patience & Gitmerge-resolve \\
\midrule
Gitmerge-ort & - & 1 & 0 & 1 & 1 & 0 & 2 \\
Gitmerge-ort-ignorespace & 6 & - & 6 & 7 & 7 & 6 & 8 \\
Gitmerge-recursive-histogram & 0 & 1 & - & 1 & 1 & 0 & 2 \\
Gitmerge-recursive-minimal & 1 & 2 & 1 & - & 0 & 0 & 1 \\
Gitmerge-recursive-myers & 1 & 2 & 1 & 0 & - & 0 & 1 \\
Gitmerge-recursive-patience & 1 & 2 & 1 & 1 & 1 & - & 2 \\
Gitmerge-resolve & 1 & 2 & 1 & 0 & 0 & 0 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/greatest_hits/tables/tools/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  54\% &  32\% &  42\% &  66\% &   4\% &   2\% \\
            Gitmerge-ort-ignorespace         &  55\% &  34\% &  41\% &  63\% &   4\% &   3\% \\
            Hires-Merge                      &  59\% &  40\% &  36\% &  56\% &   6\% &   4\% \\
            Spork                            &  58\% &  44\% &  26\% &  50\% &  16\% &   6\% \\
            IntelliMerge                     &  25\% &  15\% &  19\% &  40\% &  56\% &  46\% \\
            Adjacent                         &  59\% &  40\% &  36\% &  57\% &   6\% &   3\% \\
            Imports                          &  57\% &  35\% &  39\% &  62\% &   4\% &   3\% \\
            Version Numbers                  &  54\% &  32\% &  41\% &  65\% &   4\% &   2\% \\
            IVn                              &  58\% &  36\% &  38\% &  61\% &   4\% &   3\% \\
            IVn-ignorespace                  &  59\% &  37\% &  38\% &  59\% &   3\% &   4\% \\
\end{tabular}


==> results/greatest_hits/tables/tools/table_summary.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{l|c c|c c|c c|}
        Tool & \multicolumn{6}{c|}{Merges} \\ \cline{2-7}
        & \multicolumn{2}{c|}{Correct} &
        \multicolumn{2}{c|}{Unhandled} &
        \multicolumn{2}{c|}{Incorrect} \\
        & \# & \% & \# & \% & \# & \% \\
        \hline
Gitmerge-ort                     &   483 &  42\% &   631 &  55\% &    35 &   3\% \\
Gitmerge-ort-ignorespace         &   499 &  43\% &   612 &  53\% &    38 &   3\% \\
Hires-Merge                      &   554 &  48\% &   541 &  47\% &    54 &   5\% \\
Spork                            &   579 &  50\% &   451 &  39\% &   119 &  10\% \\
IntelliMerge                     &   223 &  19\% &   347 &  30\% &   579 &  50\% \\
Adjacent                         &   556 &  48\% &   542 &  47\% &    51 &   4\% \\
Imports                          &   512 &  45\% &   597 &  52\% &    40 &   3\% \\
Version Numbers                  &   487 &  42\% &   627 &  55\% &    35 &   3\% \\
IVn                              &   530 &  46\% &   579 &  50\% &    40 &   3\% \\
IVn-ignorespace                  &   540 &  47\% &   565 &  49\% &    44 &   4\% \\
\end{tabular}


==> results/greatest_hits/tables/tools/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Hires-Merge & Spork & IntelliMerge & Adjacent & Imports & Version Numbers & IVn & IVn-ignorespace \\
\midrule
Gitmerge-ort & - & 1 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-ort-ignorespace & 6 & - & 5 & 3 & 1 & 5 & 6 & 6 & 5 & 0 \\
Hires-Merge & 20 & 18 & - & 9 & 9 & 13 & 19 & 20 & 19 & 17 \\
Spork & 48 & 46 & 38 & - & 8 & 34 & 41 & 48 & 41 & 39 \\
IntelliMerge & 313 & 300 & 262 & 157 & - & 253 & 283 & 313 & 273 & 263 \\
Adjacent & 16 & 16 & 10 & 7 & 4 & - & 16 & 16 & 15 & 15 \\
Imports & 0 & 1 & 1 & 0 & 3 & 0 & - & 0 & 0 & 1 \\
Version Numbers & 0 & 1 & 1 & 0 & 1 & 0 & 0 & - & 0 & 1 \\
IVn & 0 & 1 & 1 & 0 & 3 & 0 & 0 & 0 & - & 1 \\
IVn-ignorespace & 7 & 0 & 6 & 4 & 4 & 6 & 7 & 7 & 6 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/reaper/defs.tex <==
\def\reaperReposInitial{25776\xspace}
\def\reaperReposValid{3977\xspace}
\def\reaperMergesInitial{205585\xspace}
\def\reaperMergesPer{100\xspace}
\def\reaperMergesNonTrivial{75517\xspace}
\def\reaperReposNonTrivial{2622\xspace}
\def\reaperMergesJavaDiff{19876\xspace}
\def\reaperReposJavaDiff{1578\xspace}
\def\reaperMergesJavaDiffAndParentsPass{5477\xspace}
\def\reaperReposJavaDiffAndParentsPass{1061\xspace}
\def\reaperReposSampled{1061\xspace}
\def\reaperMergesSampled{5461\xspace}
\def\reaperReposYieldedFull{2\xspace}
\def\reaperReposTotal{1058\xspace}
\def\reaperMergesTotal{5416\xspace}

% Results
\def\reaperAverageTriesUntilPass{1.014934660858743\xspace}
\def\reaperNumberofMergesWith1TriesUntilPass{82774\xspace}
\def\reaperNumberofMergesWith3TriesUntilPass{166\xspace}
\def\reaperNumberofMergesWith5TriesUntilPass{70\xspace}
\def\reaperNumberofMergesWith2TriesUntilPass{513\xspace}
\def\reaperNumberofMergesWith4TriesUntilPass{41\xspace}
\def\reaperSporkOverOrtCorrect{449\xspace}
\def\reaperSporkOverOrtIncorrect{441\xspace}
\def\reaperMainBranchMerges{3252\xspace}
\def\reaperMainBranchMergesPercent{60\xspace}
\def\reaperOtherBranchMerges{2164\xspace}
\def\reaperOtherBranchMergesPercent{40\xspace}
\def\reaperReposJava{25776\xspace}

% Timeout
\def\reaperParentTestTimeout{30\xspace}
\def\reaperMergeTestTimeout{45\xspace}


==> results/reaper/tables/all/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-ort-ignorespace         &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Gitmerge-recursive-histogram     &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-recursive-myers-ignorespace &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Gitmerge-recursive-minimal       &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-recursive-myers         &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-recursive-patience      &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-resolve                 &  53\% &  35\% &  45\% &  62\% &   3\% &   3\% \\
            Hires-Merge                      &  57\% &  41\% &  39\% &  55\% &   4\% &   4\% \\
            Spork                            &  62\% &  43\% &  28\% &  45\% &  10\% &  12\% \\
            IntelliMerge                     &  27\% &  19\% &  21\% &  34\% &  52\% &  47\% \\
            Adjacent                         &  58\% &  42\% &  38\% &  54\% &   4\% &   4\% \\
            Imports                          &  56\% &  39\% &  41\% &  58\% &   3\% &   3\% \\
            Version Numbers                  &  54\% &  37\% &  43\% &  61\% &   3\% &   3\% \\
            IVn                              &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            IVn-ignorespace                  &  59\% &  43\% &  37\% &  54\% &   3\% &   4\% \\
            Gitmerge-ort-plus                &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Gitmerge-ort-ignorespace-plus    &  59\% &  43\% &  37\% &  54\% &   3\% &   4\% \\
            Gitmerge-recursive-histogram-plus &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Gitmerge-recursive-myers-ignorespace-plus &  59\% &  43\% &  37\% &  54\% &   3\% &   4\% \\
            Gitmerge-recursive-minimal-plus  &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Gitmerge-recursive-myers-plus    &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Gitmerge-recursive-patience-plus &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Gitmerge-resolve-plus            &  57\% &  41\% &  41\% &  57\% &   3\% &   3\% \\
            Git-hires-merge-plus             &  61\% &  46\% &  35\% &  50\% &   4\% &   4\% \\
            Spork-plus                       &  64\% &  47\% &  26\% &  42\% &  11\% &  12\% \\
            Intellimerge-plus                &   8\% &   9\% &  20\% &  33\% &  71\% &  58\% \\
            Adjacent-plus                    &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Imports-plus                     &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Version-numbers-plus             &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Ivn-plus                         &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            Ivn-ignorespace-plus             &  59\% &  43\% &  37\% &  54\% &   3\% &   4\% \\
\end{tabular}


==> results/reaper/tables/all/table_summary.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{l|c c|c c|c c|}
        Tool & \multicolumn{6}{c|}{Merges} \\ \cline{2-7}
        & \multicolumn{2}{c|}{Correct} &
        \multicolumn{2}{c|}{Unhandled} &
        \multicolumn{2}{c|}{Incorrect} \\
        & \# & \% & \# & \% & \# & \% \\
        \hline
Gitmerge-ort                     &  2513 &  46\% &  2759 &  51\% &   144 &   3\% \\
Gitmerge-ort-ignorespace         &  2648 &  49\% &  2593 &  48\% &   175 &   3\% \\
Gitmerge-recursive-histogram     &  2513 &  46\% &  2759 &  51\% &   144 &   3\% \\
Gitmerge-recursive-myers-ignorespace &  2649 &  49\% &  2589 &  48\% &   178 &   3\% \\
Gitmerge-recursive-minimal       &  2513 &  46\% &  2758 &  51\% &   145 &   3\% \\
Gitmerge-recursive-myers         &  2513 &  46\% &  2758 &  51\% &   145 &   3\% \\
Gitmerge-recursive-patience      &  2515 &  46\% &  2756 &  51\% &   145 &   3\% \\
Gitmerge-resolve                 &  2473 &  46\% &  2799 &  52\% &   144 &   3\% \\
Hires-Merge                      &  2754 &  51\% &  2461 &  45\% &   201 &   4\% \\
Spork                            &  2962 &  55\% &  1869 &  35\% &   585 &  11\% \\
IntelliMerge                     &  1294 &  24\% &  1408 &  26\% &  2714 &  50\% \\
Adjacent                         &  2793 &  52\% &  2424 &  45\% &   199 &   4\% \\
Imports                          &  2658 &  49\% &  2607 &  48\% &   151 &   3\% \\
Version Numbers                  &  2545 &  47\% &  2727 &  50\% &   144 &   3\% \\
IVn                              &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
IVn-ignorespace                  &  2856 &  53\% &  2377 &  44\% &   183 &   3\% \\
Gitmerge-ort-plus                &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
Gitmerge-ort-ignorespace-plus    &  2856 &  53\% &  2377 &  44\% &   183 &   3\% \\
Gitmerge-recursive-histogram-plus &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
Gitmerge-recursive-myers-ignorespace-plus &  2855 &  53\% &  2376 &  44\% &   185 &   3\% \\
Gitmerge-recursive-minimal-plus  &  2755 &  51\% &  2509 &  46\% &   152 &   3\% \\
Gitmerge-recursive-myers-plus    &  2755 &  51\% &  2509 &  46\% &   152 &   3\% \\
Gitmerge-recursive-patience-plus &  2756 &  51\% &  2509 &  46\% &   151 &   3\% \\
Gitmerge-resolve-plus            &  2724 &  50\% &  2543 &  47\% &   149 &   3\% \\
Git-hires-merge-plus             &  2971 &  55\% &  2235 &  41\% &   210 &   4\% \\
Spork-plus                       &  3087 &  57\% &  1737 &  32\% &   592 &  11\% \\
Intellimerge-plus                &   465 &   9\% &  1370 &  25\% &  3581 &  66\% \\
Adjacent-plus                    &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
Imports-plus                     &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
Version-numbers-plus             &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
Ivn-plus                         &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
Ivn-ignorespace-plus             &  2856 &  53\% &  2377 &  44\% &   183 &   3\% \\
\end{tabular}


==> results/reaper/tables/all/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Gitmerge-recursive-histogram & Gitmerge-recursive-myers-ignorespace & Gitmerge-recursive-minimal & Gitmerge-recursive-myers & Gitmerge-recursive-patience & Gitmerge-resolve & Hires-Merge & Spork & IntelliMerge & Adjacent & Imports & Version Numbers & IVn & IVn-ignorespace & Gitmerge-ort-plus & Gitmerge-ort-ignorespace-plus & Gitmerge-recursive-histogram-plus & Gitmerge-recursive-myers-ignorespace-plus & Gitmerge-recursive-minimal-plus & Gitmerge-recursive-myers-plus & Gitmerge-recursive-patience-plus & Gitmerge-resolve-plus & Git-hires-merge-plus & Spork-plus & Intellimerge-plus & Adjacent-plus & Imports-plus & Version-numbers-plus & Ivn-plus & Ivn-ignorespace-plus \\
\midrule
Gitmerge-ort & - & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 5 & 8 & 0 & 0 & 0 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 12 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-ort-ignorespace & 26 & - & 26 & 0 & 26 & 26 & 26 & 28 & 21 & 20 & 18 & 18 & 26 & 26 & 25 & 0 & 25 & 0 & 25 & 0 & 25 & 25 & 25 & 27 & 19 & 18 & 23 & 25 & 25 & 25 & 25 & 0 \\
Gitmerge-recursive-histogram & 0 & 2 & - & 2 & 0 & 0 & 0 & 2 & 0 & 5 & 8 & 0 & 0 & 0 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 12 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-recursive-myers-ignorespace & 28 & 1 & 28 & - & 27 & 27 & 27 & 30 & 22 & 22 & 18 & 20 & 26 & 28 & 25 & 0 & 25 & 0 & 25 & 0 & 25 & 25 & 25 & 28 & 19 & 19 & 23 & 25 & 25 & 25 & 25 & 0 \\
Gitmerge-recursive-minimal & 1 & 3 & 1 & 2 & - & 0 & 0 & 2 & 0 & 5 & 8 & 1 & 0 & 1 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 12 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-recursive-myers & 1 & 3 & 1 & 2 & 0 & - & 0 & 2 & 0 & 5 & 8 & 1 & 0 & 1 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 12 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-recursive-patience & 1 & 3 & 1 & 2 & 0 & 0 & - & 2 & 0 & 5 & 8 & 1 & 0 & 1 & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 12 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-resolve & 2 & 4 & 2 & 3 & 1 & 1 & 1 & - & 1 & 6 & 8 & 2 & 1 & 2 & 1 & 3 & 1 & 3 & 1 & 3 & 1 & 1 & 1 & 0 & 1 & 4 & 12 & 1 & 1 & 1 & 1 & 3 \\
Hires-Merge & 57 & 53 & 57 & 52 & 56 & 56 & 56 & 58 & - & 29 & 23 & 37 & 56 & 56 & 53 & 49 & 53 & 49 & 53 & 49 & 53 & 53 & 53 & 56 & 0 & 23 & 26 & 53 & 53 & 53 & 53 & 49 \\
Spork & 262 & 242 & 262 & 241 & 261 & 261 & 259 & 267 & 214 & - & 68 & 214 & 233 & 258 & 224 & 202 & 224 & 202 & 224 & 201 & 223 & 223 & 222 & 229 & 176 & 0 & 70 & 224 & 224 & 224 & 224 & 202 \\
IntelliMerge & 1393 & 1288 & 1393 & 1286 & 1391 & 1391 & 1387 & 1405 & 1167 & 676 & - & 1142 & 1276 & 1392 & 1230 & 1151 & 1230 & 1151 & 1230 & 1152 & 1228 & 1228 & 1226 & 1244 & 1023 & 621 & 5 & 1230 & 1230 & 1230 & 1230 & 1151 \\
Adjacent & 55 & 50 & 55 & 50 & 55 & 55 & 54 & 57 & 35 & 31 & 23 & - & 49 & 55 & 49 & 44 & 49 & 44 & 49 & 44 & 49 & 49 & 48 & 51 & 29 & 27 & 26 & 49 & 49 & 49 & 49 & 44 \\
Imports & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & - & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & 0 & 0 & 0 & 0 & 1 \\
Version Numbers & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 5 & 8 & 0 & 0 & - & 0 & 2 & 0 & 2 & 0 & 2 & 0 & 0 & 0 & 2 & 0 & 3 & 12 & 0 & 0 & 0 & 0 & 2 \\
IVn & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & - & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & 0 & 0 & 0 & 0 & 1 \\
IVn-ignorespace & 26 & 0 & 26 & 1 & 26 & 26 & 26 & 30 & 21 & 22 & 22 & 19 & 26 & 26 & 25 & - & 25 & 0 & 25 & 1 & 25 & 25 & 25 & 29 & 19 & 19 & 27 & 25 & 25 & 25 & 25 & 0 \\
Gitmerge-ort-plus & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & - & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-ort-ignorespace-plus & 26 & 0 & 26 & 1 & 26 & 26 & 26 & 30 & 21 & 22 & 22 & 19 & 26 & 26 & 25 & 0 & 25 & - & 25 & 1 & 25 & 25 & 25 & 29 & 19 & 19 & 27 & 25 & 25 & 25 & 25 & 0 \\
Gitmerge-recursive-histogram-plus & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & - & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-recursive-myers-ignorespace-plus & 28 & 1 & 28 & 0 & 27 & 27 & 28 & 32 & 22 & 24 & 22 & 21 & 27 & 28 & 26 & 1 & 26 & 1 & 26 & - & 25 & 25 & 26 & 30 & 19 & 20 & 27 & 26 & 26 & 26 & 26 & 1 \\
Gitmerge-recursive-minimal-plus & 1 & 2 & 1 & 2 & 0 & 0 & 1 & 4 & 0 & 8 & 12 & 1 & 1 & 1 & 1 & 2 & 1 & 2 & 1 & 2 & - & 0 & 1 & 4 & 0 & 5 & 16 & 1 & 1 & 1 & 1 & 2 \\
Gitmerge-recursive-myers-plus & 1 & 2 & 1 & 2 & 0 & 0 & 1 & 4 & 0 & 8 & 12 & 1 & 1 & 1 & 1 & 2 & 1 & 2 & 1 & 2 & 0 & - & 1 & 4 & 0 & 5 & 16 & 1 & 1 & 1 & 1 & 2 \\
Gitmerge-recursive-patience-plus & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & - & 4 & 0 & 4 & 16 & 0 & 0 & 0 & 0 & 1 \\
Gitmerge-resolve-plus & 2 & 3 & 2 & 3 & 1 & 1 & 2 & 0 & 1 & 9 & 11 & 2 & 2 & 2 & 2 & 3 & 2 & 3 & 2 & 3 & 1 & 1 & 2 & - & 1 & 6 & 15 & 2 & 2 & 2 & 2 & 3 \\
Git-hires-merge-plus & 59 & 53 & 59 & 53 & 58 & 58 & 59 & 62 & 0 & 33 & 27 & 36 & 59 & 58 & 56 & 50 & 56 & 50 & 56 & 50 & 55 & 55 & 56 & 60 & - & 26 & 30 & 56 & 56 & 56 & 56 & 50 \\
Spork-plus & 267 & 245 & 267 & 245 & 267 & 267 & 265 & 274 & 218 & 0 & 73 & 219 & 246 & 263 & 238 & 213 & 238 & 213 & 238 & 212 & 237 & 237 & 236 & 244 & 188 & - & 75 & 238 & 238 & 238 & 238 & 213 \\
Intellimerge-plus & 1391 & 1291 & 1391 & 1289 & 1390 & 1390 & 1386 & 1419 & 1172 & 691 & 0 & 1140 & 1274 & 1390 & 1228 & 1154 & 1228 & 1154 & 1228 & 1155 & 1227 & 1227 & 1225 & 1251 & 1025 & 634 & - & 1228 & 1228 & 1228 & 1228 & 1154 \\
Adjacent-plus & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & - & 0 & 0 & 0 & 1 \\
Imports-plus & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & 0 & - & 0 & 0 & 1 \\
Version-numbers-plus & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & 0 & 0 & - & 0 & 1 \\
Ivn-plus & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 7 & 12 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 2 & 0 & 0 & 0 & 4 & 0 & 4 & 16 & 0 & 0 & 0 & - & 1 \\
Ivn-ignorespace-plus & 26 & 0 & 26 & 1 & 26 & 26 & 26 & 30 & 21 & 22 & 22 & 19 & 26 & 26 & 25 & 0 & 25 & 0 & 25 & 1 & 25 & 25 & 25 & 29 & 19 & 19 & 27 & 25 & 25 & 25 & 25 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/reaper/tables/git/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-ort-ignorespace         &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Gitmerge-recursive-histogram     &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-recursive-minimal       &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-recursive-myers         &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-recursive-patience      &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-resolve                 &  53\% &  35\% &  45\% &  62\% &   3\% &   3\% \\
\end{tabular}


==> results/reaper/tables/git/table_summary.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{l|c c|c c|c c|}
        Tool & \multicolumn{6}{c|}{Merges} \\ \cline{2-7}
        & \multicolumn{2}{c|}{Correct} &
        \multicolumn{2}{c|}{Unhandled} &
        \multicolumn{2}{c|}{Incorrect} \\
        & \# & \% & \# & \% & \# & \% \\
        \hline
Gitmerge-ort                     &  2513 &  46\% &  2759 &  51\% &   144 &   3\% \\
Gitmerge-ort-ignorespace         &  2648 &  49\% &  2593 &  48\% &   175 &   3\% \\
Gitmerge-recursive-histogram     &  2513 &  46\% &  2759 &  51\% &   144 &   3\% \\
Gitmerge-recursive-minimal       &  2513 &  46\% &  2758 &  51\% &   145 &   3\% \\
Gitmerge-recursive-myers         &  2513 &  46\% &  2758 &  51\% &   145 &   3\% \\
Gitmerge-recursive-patience      &  2515 &  46\% &  2756 &  51\% &   145 &   3\% \\
Gitmerge-resolve                 &  2473 &  46\% &  2799 &  52\% &   144 &   3\% \\
\end{tabular}


==> results/reaper/tables/git/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Gitmerge-recursive-histogram & Gitmerge-recursive-minimal & Gitmerge-recursive-myers & Gitmerge-recursive-patience & Gitmerge-resolve \\
\midrule
Gitmerge-ort & - & 2 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-ort-ignorespace & 26 & - & 26 & 26 & 26 & 26 & 28 \\
Gitmerge-recursive-histogram & 0 & 2 & - & 0 & 0 & 0 & 2 \\
Gitmerge-recursive-minimal & 1 & 3 & 1 & - & 0 & 0 & 2 \\
Gitmerge-recursive-myers & 1 & 3 & 1 & 0 & - & 0 & 2 \\
Gitmerge-recursive-patience & 1 & 3 & 1 & 0 & 0 & - & 2 \\
Gitmerge-resolve & 2 & 4 & 2 & 1 & 1 & 1 & - \\
\bottomrule
\end{tabular}
\end{table}


==> results/reaper/tables/tools/table_feature_main_summary.tex <==
% Do not edit.  This file is automatically generated.
\setlength{\tabcolsep}{.285\tabcolsep}
\begin{tabular}{c|cc|cc|cc}
            Tool &
            \multicolumn{6}{c}{Merges} \\ \cline{2-7}
            &
            \multicolumn{2}{c|}{Correct} &
            \multicolumn{2}{c|}{Unhandled} &
            \multicolumn{2}{c}{Incorrect} \\
            &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c|}{Other} &
            \multicolumn{1}{c}{Main} &
            \multicolumn{1}{c}{Other} \\
            \hline
            Gitmerge-ort                     &  54\% &  36\% &  44\% &  62\% &   3\% &   3\% \\
            Gitmerge-ort-ignorespace         &  56\% &  38\% &  41\% &  59\% &   3\% &   3\% \\
            Hires-Merge                      &  57\% &  41\% &  39\% &  55\% &   4\% &   4\% \\
            Spork                            &  62\% &  43\% &  28\% &  45\% &  10\% &  12\% \\
            IntelliMerge                     &  27\% &  19\% &  21\% &  34\% &  52\% &  47\% \\
            Adjacent                         &  58\% &  42\% &  38\% &  54\% &   4\% &   4\% \\
            Imports                          &  56\% &  39\% &  41\% &  58\% &   3\% &   3\% \\
            Version Numbers                  &  54\% &  37\% &  43\% &  61\% &   3\% &   3\% \\
            IVn                              &  57\% &  41\% &  40\% &  56\% &   3\% &   3\% \\
            IVn-ignorespace                  &  59\% &  43\% &  37\% &  54\% &   3\% &   4\% \\
\end{tabular}


==> results/reaper/tables/tools/table_summary.tex <==
% Do not edit.  This file is automatically generated.
\begin{tabular}{l|c c|c c|c c|}
        Tool & \multicolumn{6}{c|}{Merges} \\ \cline{2-7}
        & \multicolumn{2}{c|}{Correct} &
        \multicolumn{2}{c|}{Unhandled} &
        \multicolumn{2}{c|}{Incorrect} \\
        & \# & \% & \# & \% & \# & \% \\
        \hline
Gitmerge-ort                     &  2513 &  46\% &  2759 &  51\% &   144 &   3\% \\
Gitmerge-ort-ignorespace         &  2648 &  49\% &  2593 &  48\% &   175 &   3\% \\
Hires-Merge                      &  2754 &  51\% &  2461 &  45\% &   201 &   4\% \\
Spork                            &  2962 &  55\% &  1869 &  35\% &   585 &  11\% \\
IntelliMerge                     &  1294 &  24\% &  1408 &  26\% &  2714 &  50\% \\
Adjacent                         &  2793 &  52\% &  2424 &  45\% &   199 &   4\% \\
Imports                          &  2658 &  49\% &  2607 &  48\% &   151 &   3\% \\
Version Numbers                  &  2545 &  47\% &  2727 &  50\% &   144 &   3\% \\
IVn                              &  2755 &  51\% &  2510 &  46\% &   151 &   3\% \\
IVn-ignorespace                  &  2856 &  53\% &  2377 &  44\% &   183 &   3\% \\
\end{tabular}


==> results/reaper/tables/tools/tool_comparison_table.tex <==
% Do not edit. This file is automatically generated.
\begin{table}[h]
\centering
\caption{Comparison of Merge Tool Results: Incorrect vs Unhandled}
\label{tab:tool-comparison}
\small
\begin{tabular}{lrrrrrrrrrr}
\toprule
& Gitmerge-ort & Gitmerge-ort-ignorespace & Hires-Merge & Spork & IntelliMerge & Adjacent & Imports & Version Numbers & IVn & IVn-ignorespace \\
\midrule
Gitmerge-ort & - & 2 & 0 & 5 & 8 & 0 & 0 & 0 & 0 & 2 \\
Gitmerge-ort-ignorespace & 26 & - & 21 & 20 & 18 & 18 & 26 & 26 & 25 & 0 \\
Hires-Merge & 57 & 53 & - & 29 & 23 & 37 & 56 & 56 & 53 & 49 \\
Spork & 262 & 242 & 214 & - & 68 & 214 & 233 & 258 & 224 & 202 \\
IntelliMerge & 1393 & 1288 & 1167 & 676 & - & 1142 & 1276 & 1392 & 1230 & 1151 \\
Adjacent & 55 & 50 & 35 & 31 & 23 & - & 49 & 55 & 49 & 44 \\
Imports & 0 & 1 & 0 & 7 & 12 & 0 & - & 0 & 0 & 1 \\
Version Numbers & 0 & 2 & 0 & 5 & 8 & 0 & 0 & - & 0 & 2 \\
IVn & 0 & 1 & 0 & 7 & 12 & 0 & 0 & 0 & - & 1 \\
IVn-ignorespace & 26 & 0 & 21 & 22 & 22 & 19 & 26 & 26 & 25 & - \\
\bottomrule
\end{tabular}
\end{table}

